Multi-Agent Contract Design beyond Binary Actions

We study hidden-action principal-agent problems with multiple agents. Unlike previous work, we consider a general setting in which each agent has an arbitrary number of actions, and the joint action induces outcomes according to an arbitrary distribution. We study two classes of mechanisms: a class of deterministic mechanisms that is the natural extension of single-agent contracts, in which the agents play a Nash equilibrium of the game induced by the contract, and a class of randomized mechanisms that is inspired by single-agent randomized contracts and correlated equilibria.

==> src/intro_v1.tex <==
\section{Introduction}\label{sec:intro}

Over the last years, contract design has received a growing attention as a tool to model the interaction between a \emph{principal} and one or multiple \emph{agents}. The principal’s objective is to incentivize the agents to undertake costly actions that lead to desirable outcomes.
Our work focuses on hidden-action problems, where the principal can only observe an outcome stochastically determined by the agents’ actions, but not the actions themselves.
To steer the agents' behavior, the principal designs a \emph{contract}, that specifies outcome-dependent payments to the agents.
Such principal-agent interactions are ubiquitous in real-world scenarios such as crowdsourcing platforms~\citep{ho2016adaptive}, blockchain-based smart contracts~\citep{cong2019blockchain}, and healthcare~\citep{bastani2016analysis}.


The computational study of principal-agent problems involving a single agent has been widely investigated in the literature. The vanilla version of this problem can be solved in polynomial time via multiple linear programs~ \citep{grossman1992analysis}. \citet{dutting2019simple} examine the properties of linear contracts. Some works studies more complex Bayesian settings in which agent have types~\cite{castiglioni2022bayesian,castiglioni2023designing, alon2021contracts, alon2023bayesian,GuruganeshPower23,guruganesh2021contracts}, while other works extends the model to include combinatorial actions~\citep{dutting2021complexity,dutting2022combinatorial,dutting2024combinatorial}.
%

A natural extension of this model involves a scenario where a principal has to incentivize a \emph{team} of agents~\citep{holmstrom1982moral}. This problem introduces additional challenges due to inherently combinatorial structure of the problem. 
Most works focus on succinct representations and binary actions~\citep{babaioff2012combinatorial, emek2012computing,dutting2023multi,deo2024supermodular}. In particular, each agent chooses only between exerting or not exerting an effort.
A notable exception is \citep{castiglioni23multi}, which study a setting with arbitrary action sets but limited externalities among the agents.

Surprisingly, the general problem of incentivizing multiple agents has been largely neglected. Here, we focus on the natural extension of the single-agent principal-agent problem, where each agent has an arbitrary number of actions, and the outcome is sampled from an arbitrary probability distribution determined by the joint action of the agents.
%
Considering this non-succinct multi-agent problem trivializes the computational challenge of computing an optimal contract. Indeed, it can be computed in polynomial time by solving an linear problem for each action profile, similarly to single-agent contracts~\citep{grossman1992analysis}. However, there are many other questions that deserve an answer. In this works, we focus on the following:
\begin{enumerate}
	\item Are there better mechanisms than standard deterministic contracts?
	\item Which are the guarantees of  simple (\emph{e.g., linear}) contracts?
		\item How externalizes among the agents affect the principal's utility?
\end{enumerate}

 
\subsection{Our Contributions}

\mat{mettere i teoremi?}
\mat{siamo i primi che studiamo setting bayesiani con più agenti!}
We investigate the problem of finding contract in multi-agent principal-agent problems. Unlike previous work, we consider a general setting in which each agent has an arbitrary number of actions, and the joint action induces outcomes according to an arbitrary distribution.
We study two classes of mechanisms: a class of deterministic mechanisms that is the natural extension of single-agent contracts, in which the agents play a Nash equilibrium of the game induced by the contract, and a class of randomized mechanisms that is inspired by single-agent randomized contracts and correlated equilibria.
While deterministic contracts are provably optimal in single-agent (non-Bayesian) problems, we show that randomization is fundamental to design optimal multi-agent contracts. Indeed, we show that randomized mechanisms provide an arbitrarily larger principal’s utility than deterministic ones. Following, this fact, we focus on the design of a polynomial-time algorithm to compute almost optimal randomized contracts. When compared with the task of computing optimal deterministic contracts, which can be trivially addressed regardless of the number of agents, the computation of an optimal randomized contract introduces significant challenges in multi-agent problems. In this context, we first show that, in general, an optimal randomized contract may not exist, thus moving our attention to finding a randomized contract which is \emph{approximately} optimal. To do so, we provide a linear relaxation of the quadratic optimization problem that computes an optimal contract and then we show how to convert a solution to such a relaxed problem into an almost optimal randomized contract.

Subsequently, we investigate which are the effects of \emph{externalities} between the agents on the principal's utility. 
%To achieve this goal we relate the principal's utility in the multi-agent instance to the single-agent instance with combinatorial actions consisting in the joint actions.
%We formalize the intuition that incentivize multiple agents is harder than a single one and the gap between the principal's utility in the multi-agent instance is arbitrary small than in the single-agent one.
%
%However, we show that the formalize and quantify this intuition through virtual cost.
%In particular, we show that moving from the single-agent problem to a multi-agent one is ‘‘no worse'' than increasing the costs by an $n$ factor where $n$ is the number of agents, and that this factor is tight.
%Leveraging this result, we obtain that, for any $\delta\ge 0$, the optimal deterministic contract extracts a constant fraction $\delta/(1+\delta)$ of the  social welfare of a virtual  instance in which costs are increased by a $(1+\delta) n$ factor. 
%Our result is constructive and shows how to recover a multi-agent deterministic contract from a contract for the virtual single-agent instance. Moreover, enjoy the property of being a simple linear contract.
%At the core of our analysis is the relation among the best response to a contract of a single agent and the equilibria in the multi-agent problem induced by the contract.
%
We tackle this problem by relating our multi-agent problem to a single-agent instance in which the actions available to the agent are the joint actions of the agents in the multi-agent instance. Given that the single-agent instance is defined to be in fact equivalent to the multi-agent instance, except for the fact that in the former all inter-agents externalities are missing, this connection allows us to determine exactly the effect of such externalities in the utility of the principal. 
%Interestingly, leveraging the concept of \emph{virtual costs}, our analysis shows that the utility for the principal in the instance with $n$ agents is at least the utility of the principal in the single-agent instance in which the costs are increased by a $n$ factor, and that this result is tight in its dependency from $n$. 
Interestingly, leveraging the concept of \emph{virtual costs}, our analysis shows that moving from a $n$-agent instance to the associated single-agent one is ‘‘no worse'' than increasing the costs by an $n$ factor where $n$ is the number of agents, and that this factor is tight. In other words, this suggests that the presence of externalities causes an increase in the virtual costs by a factor $n$. Moreover, building on this result, we were able to show that for any $\delta\ge 0$, the optimal deterministic contract extracts a constant fraction $\delta/(1+\delta)$ of the  social welfare of a virtual  instance in which costs are increased by a $(1+\delta) n$ factor. Our result is constructive and shows how to recover a multi-agent deterministic contract from a simple \emph{linear} contract for the virtual single-agent instance.
 
In the second part of the paper, we investigate whether our results carry over the more complex Bayesian setting with typed agents. We show that our computational result on randomized contract extends to this setting, and an almost optimal randomized contract can be computed in polynomial time. Notice that this is not the case for deterministic contracts, for which the problem is NP-Hard even in single-agent problems~\cite{castiglioni2022bayesian,guruganesh2021contracts}. This computational aspects further motivates the study of the performances of simple deterministic contracts that can be computed efficiently.
%However, we prove that our reduction between single- and multi-agent contracts does not extend to Bayesian settings.
%Indeed, we provide an instance in which an optimal deterministic contract cannot extract any fraction of the virtual social welfare for any choice of the virtual costs.
%Nonetheless, we show that this impossibility result can be circumvented by removing limited liability.
%We highlight that while in single-agent non-Bayesian setting trivialized the contract design problem and a simple contract guarantees to the principal to extract all the social welfare, this is not the case in our setting. Indeed, we show that the gap between the optimal principal's utility and the social welfare is arbitrarily large.
%We design a mechanism that does not guarantee limited liability but extracts exactly the same approximation of the virtual social welfare as in non-Bayesian settings. Here, while this task is unachievable with linear contracts (notice that they satisfy limited liability), we show that we can do it with affine contracts that are composed by a linear contract and a outcome-independent constant negative payment .
%We conclude by showing that in Bayesian settings with single-dimensional types our result extends to the (non-virtual) social welfare under reasonable assumptions. This generalizes the results from \citet{alon2023bayesian} to multi-agents settings.
Unfortunately, we prove that our reduction between single- and multi-agent contracts does not extend to Bayesian settings even when the types are \emph{single-dimensional}. Indeed, we provide an instance in which an optimal deterministic contract cannot extract any fraction of the virtual social welfare for any choice of the virtual costs. Nonetheless, we show that this impossibility result can be circumvented by removing limited liability. In particular, we design a mechanism that does not guarantee limited liability but extracts exactly the same approximation of the virtual social welfare as in non-Bayesian settings. Notice that, in light of our negative result, this task cannot be achieved by a mere linear contract (as it would satisfy limited liability by construction), but we show that it is possible to use an \emph{affine} contract, composed by a linear contract and a and an outcome-independent constant negative payment. We conclude by showing that in Bayesian settings with single-dimensional types our result extends to the (non-virtual) social welfare under reasonable assumptions. This generalizes the results from \citet{alon2023bayesian} to multi-agents settings.

\fe{C'era questa frase qui ma non l'ho troppo capita}\fe{We highlight that, while in single-agent non-Bayesian setting trivialized the contract design problem and a simple contract guarantees to the principal to extract all the social welfare, this is not the case in our setting. Indeed, we show that the gap between the optimal principal's utility and the social welfare is arbitrarily large.} 

\subsection{Related Works}

We survey the most-related computational works on hidden-action principal-agent problems.

\paragraph{Works on Single-Agent Contract Design}

\cite{babaioff2014contract} study the complexity of contracts in terms of the number of different payments that they specify, while \cite{dutting2019simple} use the computational lens to analyze the efficiency (in terms of principal’s expected utility) of linear contracts with respect to optimal ones.
%
Some works focuses on the Bayesian setting. \cite{guruganesh2021contracts, GuruganeshPower23} study the gap in power between different classes of contracts. \cite{castiglioni2022bayesian} studies linear contracts in Bayesian settings. \cite{alon2021contracts,alon2023bayesian} study one-dimensional typed
principal-agent problem where the cost scales linearly with the hidden type. 
 \citet{castiglioni2023designing} introduce the class of menus of randomized contracts and show that they can be computed efficiently.
\citet{gan2022optimal} study a generalization of the principal-agent problem, proving that optimal randomized mechanisms can be computed efficiently.
Other works studies principal-agent problem in which the underlying structure is combinatorial. In particular, \cite{dutting2021complexity}  address settings in which the agent selects a subset of actions. \cite{dutting2022combinatorial} focus on submodular settings, while \cite{deo2024supermodular,dutting2024combinatorial} on supermodular functions.


\paragraph{Works on Multi-Agent Contract Design}

All the previous works on multi-agent contract design focuses on non-Bayesian settings and succinct representations. \cite{babaioff2012combinatorial,emek2012computing} are the first to study a setting in which agents have binary actions, and each agent succeeds in his task with a probability that depends on whether they decide to undertake effort. Then, a function maps the success of individual tasks to the success of the project.
individual successes and failures to a success or failure of the project. \cite{dutting2023multi} provides a constant factor approximation  for submodular rewards, while \cite{deo2024supermodular} focuses on supermodular setting providing both positive and negative results.

==> src/rcvsdc.tex <==
\section{Randomized versus Deterministic Contracts}\label{sec:rcvsdc}
%
We start our analysis by comparing the performances of randomized contracts and deterministic contracts.
%
In particular, we show that deterministic contracts constitute a more restrictive contract model for the principal, resulting in a potentially infinite gap between the utility achieved by an optimal deterministic contract and the one achieved by an optimal randomized contract. The following proposition formalizes this statement. 
%

%\mat{in generale sono un pò dubbioso sul fatto di avere questa proof nel main. Non sono troppi conti?}
\begin{restatable}{proposition}{propgap}\label{prop:propgap}
	There exists an instance of the principal-multi-agent problem in which $\frac{\optcrc}{\optdc} = \infty$.
\end{restatable}
%
\begin{proof}
	Consider an instance of the principal-multi-agent problem where $N=\{1,2\}$,  $\Omega=\{\omega_1,\omega_2\}$, and $A_1=A_2=\{\aone,\atwo\}$. The rewards are defined such that $r_{\omega_1} = 1$ and $r_{\omega_2} = 0$. The outcome probabilities are defined as in the following table: 
	%
	\begin{table}[H]
		\centering
		\begin{tabular}{|c | c c |}
			\hline 
			$F_a(\omega)$ & $\omega_1$ & $\omega_2$ \\
			\hline
			$\aone\aone$ & $1$ & $0$ \\
			$\aone\atwo$ & $2/5$ & $3/5$ \\
			$\atwo\aone$ & $2/5$ & $3/5$ \\
			$\atwo\atwo$ & $0$ & $1$ \\
			\hline 
		\end{tabular}
	\end{table}
	Additionally, the action costs are $c_i(\aone) = 2/5$ and $c_i(\atwo) = 0$ for all $i\in N$. To prove the proposition, we first show that in the consider instance the utility of the optimal deterministic contract is $0$, and then prove that $\optcrc>0$. 
	
	\paragraph{Upper bound on $\optdc$.} 
	%
	Let $(a, p)$ be an optimal deterministic contract, \emph{i.e.,} such that 
	\[
		\sum_{\omega\in\Omega} F_a(\omega) \left[r_\omega - \sum_{i\in N} p^i(\omega)\right] = \optdc.
	\]
	By  IC  with respect to action $\atwo$, the expected payment received by an agent to which is recommended action $\aone$ must be at least equal to the action cost (otherwise the agent would play $\atwo$). Formally, for each $i\in N$ such that $a_i=\aone$, it must hold that $\sum_{\omega\in\Omega} F_a(\omega) p^i(\omega) \geq c_i(\aone)$, which gives the following:
	%
	\begin{equation}\label{eq:bounddc_propgap}
		\optdc = \sum_{\omega\in\Omega} F_a(\omega) \left[r_\omega - \sum_{i\in N} p^i(\omega)\right] \leq \sum_{\omega\in\Omega} F_a(\omega)r_\omega  - \sum_{i\in N} c_i(a_i).
	\end{equation}
	%
	From \cref{eq:bounddc_propgap}, it follows that the only action profile that can achieve a strictly positive upper bound on $\optdc$ is $\aone\aone$, while all the others action profiles guarantee non-positive principal's expected utility. Hence, let us assume that the incentivized action is $a=\aone\aone$. Then, we have that the payment scheme $p$ must satisfy the following IC constraint for each $i\in N$: 
	\[
		p^i(\omega_1) - \frac{2}{5} \geq \frac{2}{5}p^i(\omega_1) + \frac{3}{5}p^i(\omega_2).
	\]
	Rearranging, we get
	\[
		\frac{3}{5}p^i(\omega_1) \ge \frac{2}{5} + \frac{3}{5}p^i(\omega_2) \ge \frac{2}{5}.
	\]
	This implies $p^i(\omega_1) \geq 2/3$ for each $i\in N$. As a consequence, we have that if a contract incentivizes action profile $\aone\aone$, then the utility for the principal must be
	\[
		\sum_{\omega\in\Omega} F_{(\aone,\aone)}(\omega) r_\omega - \sum_{i\in N} p^i(\omega) \leq 1 - \frac{4}{3} \leq 0,
	\]
	which proves that $\optdc\leq0$.
	
	\paragraph{Lower bound on $\optcrc$.} Consider the randomized contract $(\mu, \pi)$ where
	\[
		\mu(a) = \begin{cases}
			1/3 & \textnormal{if } a \neq \atwo\atwo \\
			0 &  \textnormal{if } a \neq \atwo\atwo,
		\end{cases} \quad\quad\textnormal{and}\quad\quad \pi^i_a(\omega) = \begin{cases}
		2	& \textnormal{if } a_i = \aone\,\wedge\, a_{-i}=\atwo\,\wedge\, \omega=\omega_1 \\
		0 & \textnormal{otherwise}
		\end{cases}\quad\forall i\in N.
	\]
	First, notice that the randomized contract $(\mu, \pi)$ is IC. In particular, the IC constraint when action $\aone$ is recommended to the first agent is:
	\begin{align*}
		\sum_{a_2\in A_2}& \mu(\aone, a_2) \left[U_1^{\mu, \pi}(\aone) - U_1^{\mu, \pi}(\aone\to\atwo) \right] \\
		&= \sum_{a_2\in A_2}\mu(\aone,a_2)\sum_{\omega\in\Omega} \pi^i_{(\aone, a_2)}(\omega)\left[F_{(\aone, a_2)}(\omega) - F_{(\atwo, a_2)}(\omega)\right] - \sum_{a_2\in A_2} \mu(\aone, a_2)\left[c_1(\aone) - c_1(\atwo)\right] \\
		&= \mu(\aone,\atwo)\sum_{\omega\in\Omega} \pi^1_{(\aone,\atwo)}(\omega)\left[F_{(\aone,\atwo)}(\omega) - F_{(\atwo,\atwo)}(\omega)\right] - \sum_{a_2\in A_2} \mu(\aone, a_2)\left[c_1(\aone) - c_1(\atwo)\right] \\
		&= \frac{4}{15} - \frac{4}{15} \geq 0.
	\end{align*}
	Similarly, the IC constraint is trivially satisfied when agent $i$ is recommended to play action $\atwo$, since in such a case her expected payment is $0$. This proves that $(\mu, \pi)$ is IC for agent $1$ (and hence also for agent $2$, since the agents are symmetric). To conclude the proof notice that since $(\mu, \pi)$ is a feasible contract, \emph{i.e.,} a feasible solution to \cref{prog:optrc}, the following holds: 
	\begin{align*}
		\optcrc &\ge \sum_{a\in\A}\sum_{\omega\in\Omega} \mu(a) F_a(\omega)\left[r_\omega - \sum_{i\in N} \pi^i_a(\omega)\right] = \frac{1}{3} + \frac{1}{3}\left[\frac{2}{5} - \frac{4}{5}\right] + \frac{1}{3}\left[\frac{2}{5} - \frac{4}{5}\right] = \frac{1}{15} > 0.
	\end{align*}
	This concludes the proof.
\end{proof}

The result stated in \cref{prop:propgap} highlights the relevance of randomized contracts and establishes the importance of randomization in designing optimal contracts. In the next section, we show that despite  their complexity, almost optimal randomized contracts can be computed efficiently.
